Almost Tight Approximation Hardness and Online Algorithms for Resource Scheduling

We study the precedence-constrained resource scheduling problem [SICOMP'75]. There are $n$ jobs where each job takes a certain time to finish and has a resource requirement throughout the execution time. There are precedence among the jobs. The problem asks that given a resource budget, schedule the jobs obeying the precedence constraints to minimize makespan (maximum completion time of a job) such that at any point in time, the total resource being used by all the jobs is at most the given resource budget. In the offline setting, an important open question is whether a polynomial-time $O(1)$-factor approximation algorithm can be found. We prove almost tight hardness of approximation: For some constant $\alpha > 0$, there is no $o((\log t_{\max})^{\alpha})$-factor ( or $o( ( \log n )^\alpha )$-factor ) approximation algorithm with $n$ jobs of maximum job length $t_{\max}$, unless P = NP ( or NP $\subset$ DTIME$(O( 2^{\text{polylog}(n)}))$ ). We further show a connection between this scheduling problem and a seemingly unrelated problem called the shortest common super-sequence (SCS) problem, which has wide application in Biology and Genomics. We prove that an $o(\log t_{\max})$-factor approximation of the scheduling problem would imply the existence of an $o(|\Sigma|)$-approximation algorithm for SCS with alphabet $\Sigma$. We then consider the online setting. We present $\Omega(\log n)$ and $\Omega(\log t_{\max})$ lower bounds of the competitive ratio of any randomized online algorithm. Moreover, we present a matching $O(\min\{\log n, \log t_{\max}\})$-competitive deterministic online algorithm.

==> Upper.tex <==
\section{Online Algorithm with Tight Competitive Ratio}\label{OnlineAlgSection}

In this section, we present a competitive online algorithm $\onl$.

Recall \hao{Probably don't need to say here since it's the last section probably recall?} we are given a DAG $D = (V,E)$ and $d \ge 1$ types of resource where resource $\mathcal{R}_i$ has capacity $r_i$ (after normalizing separately for each resource type, assume that each resource type has capacity $r$).
%%We are given a DAG $D = (V,E)$ and a resource capacity $r$. 
Each node $v\in V$  is a job that requires $r_{i,v}$ units of resource $\mathcal{R}_i$ for $t_v$  units of time to complete.   
For each edge $(u,v) \in E$,  we must complete job $u$ before starting job $v$. 
At any time, for each resource $\mathcal{R}_i$, we may use a total of $r$ units of resource $\mathcal{R}_i$.  \haonew{did we not rescale so there is one unit of each resource?}
The objective is to complete all jobs as soon as possible. \hao{this also needs to be in the first section?}

By losing at most a factor 2, we may round up all processing times $t_v$ to the nearest power of 2. 
%%(actually not strictly necessary but makes analysis easier).  
Henceforth, we assume all processing times are powers of 2. Also, assume that there is a single source and a single sink node in DAG $D$, otherwise, we add a dummy source and a dummy sink node to $D$.

Our main theorem of this section is as follows.
\OnlineLogApx

Before presenting the online algorithm, we define the following useful notations.

In the online setting, if all the predecessors of a job have finished their execution, the job is revealed to the online algorithm. Call a job a \defn{ready job}, if the job is not executed yet, but all of its predecessors have finished execution. For each ready job $v$, algorithm $\onl$ assigns its \defn{level} $\psi(v)$ as follows. 

\begin{definition}
Let the length of job $v$ be $2^i$. Level $\psi(v)$ is assigned as the smallest integer multiple of $2^i$ which is at least as large as $(\psi(p) + t_p)$ for all parent $p$ of job $v$. That is, 
$$
\psi(v) = \min\{k\cdot 2^i | k \in \N \text{ and }  k\cdot 2^i \ge \psi(p) + t_p  \text{ for all of } v \text{'s predecessors } p\}.
$$
\end{definition}

\paragraph{\textbf{Online algorithm ONL}} Our online algorithm $\onl$ maintains a set, called \defn{Ready-Jobs} that is the set of ready jobs. Although, any job in the set Ready-Jobs can be executed if enough resource is available for the ready job, algorithm \onl instead execute the ready jobs in a \defn{time-indexed} fashion as follows: 

\onl executes ready jobs in stages---in each stage, \onl executes only the ready jobs that are assigned the same level. If all the ready jobs that are assigned level $\ell$ have finished execution, \onl finds the next smallest level $\ell^{'} > \ell$ such that there are some ready job(s) that are assigned level $\ell^{'}$. \onl executes only the ready jobs that are assigned level $\ell^{'}$ (i.e., there could be other ready jobs sitting idle because their levels are higher than $\ell^{'}$). 

After executing level $\ell^{'}$ jobs, new jobs might be revealed and they become ready jobs. We assign level $\psi(v)$ to each new ready job $v$ and insert these new ready jobs into the set Ready-Jobs. Find the next level $\ell^{''} > \ell^{'}$, such that there is at least one ready job with level $\ell^{''}$. Execute all the jobs with level $\ell^{''}$ and then find the next non-empty level, execute those jobs, and so on. 

The algorithm finishes when there is no more ready jobs.

We present a detailed pseudocode in the full version of the paper.
\iffalse
\SetKwComment{Comment}{/* }{ */}
\begin{algorithm}[hbt!]
\caption{Online Algorithm \onl}\label{alg:two}
Ready-Jobs = $\{s\}$       \Comment*[r] {A job is ready if it is not yet executed but all its predecessors are already executed. $s$ is the source node of the DAG.}

Current-Time = 0

\While{Ready-Jobs is not empty}{
    $i$ = getNextNonEmptyLevel(Ready-Jobs)    \Comment*[r] {Find the next level $i$ such that there is a ready job that is assigned level $i$.}
    
    Working-Set$(i)$ = getJobs(Ready-Jobs, $i$)   \Comment*[r] {Working-Set$(i)$ is the set of ready jobs which are assigned level $i$.}
    
    Processing-Time = execute(Working-Set$(i)$)    \Comment*[r] {Run the jobs in Working-Set$(i)$. The function is described below.}
    
    New-Ready-Jobs = getNewReadyJobs(Ready-Jobs, Working-Set$(i)$) \Comment*[r] {Find the set of new ready jobs that reveal after executing Working-Set$(i)$.}
    
    assignLevel(New-Ready-Jobs)     \Comment*[r] {Assign level $\psi$ for each new ready job.}
    
    Ready-Jobs = ReadyJobs $\backslash$ Working-Set$(i)$ $\cup$ New-Ready-Jobs
    
    Current-Time = Current-Time + Processing-Time
    
}

Makespan = Current-Time
\end{algorithm}
\fi

\begin{definition}
For a set of jobs $W_i$ and resource type $\mathcal{R}_j$, define $\work_j(W_i) = \sum_{v \in W_i} r_{i,v} \times t_v$.
\end{definition}

We present the following upper bound of the makespan of our algorithm \onl with a detailed proof in the full version of the paper. 

Call a time-step $t$ \defn{resource efficient} during the execution of algorithm \onl, if for some resource $\mathcal{R}_j$, the total resource usage of resource $\mathcal{R}_j$ of all jobs being processed at $t$ is at least $r/2$. Otherwise, call time-step $t$ \defn{resource inefficient}. We show that the number of resource efficient time-steps is upper bounded by $2\sum_{j=1}^d \work_j(V)/r$ where $d$ is the number of resource types each with normalized capacity $r$.
To upper bound the total number of resource inefficient time-steps, we prove that all the jobs of the same length $2^i$ (without loss of generality, round each job length to the next power of $2$) together contribute  at most $\ell_{\max}$, the maximum level assigned to a job. Since there are $\log t_{\max}$ different powers of $2$ job sizes, the number of resource inefficient time-steps is at most $O(\ell_{\max} \cdot \log t_{\max})$. 
  
  %There are $\log t_{\max}$ different powers-of-$2$ job lengths, where $t_{\max}$ is the maximum job length. Thus, the total bottleneck caused by all the jobs is $O(d \cdot \log t_{\max})$. Since depth $d$ of the DAG  is a lower bound of any schedule, we get a $O(\log t_{\max})$-competitive online algorithm. 
  
To show that the number of resource inefficient time-steps is upper bounded by $O(\ell_{\max} \cdot \log |V|)$, we design a different small optimization problem based on the level assignment and the number of jobs.

\begin{lemma}\label{bdInTermstmax}
Let $V$ be the set of vertices (jobs) in the input DAG with total normalized resource capacity $r$ for each of the $d$ types of resource. Let $t_{\max}$ be the maximum job size and $\ell_{\max}$ be the maximum level a job is assigned by algorithm \onl. Then, the upper bound of makespan $T_{\onl}$ of algorithm \onl is as follows.

$$
T_{\onl} \leq 2\sum_{j=1}^d \work_j(V)/r + O(\ell_{\max} \cdot \min \{\log t_{\max}, \log |V|\}).
$$
\end{lemma}

We further prove the makespan lower bound of the optimal offline algorithm (the proof is given in the full version).
\begin{lemma}
\label{lem:opt-lower}
Let $V$ be the set of vertices (jobs) in the input DAG with total resource capacity $r$ (normalized for each resource type separately) for each resource $\mathcal{R}_i$ where $i\in[1,d]$. Let $\ell_{\max}$ be the maximum level a job is assigned by algorithm \onl. Then, the lower bound of makespan $T_{\opt}$ of the optimal algorithm \opt is as follows. \hao{You actually want $ \max_{v \in G} \phi(v) +t_v $ (-1 if you assigned the lowest level to be 1)}
$$
T_{\opt} \geq \max\Bigg(\frac{\sum_{j=1}^d \work_j(V)}{d \cdot r}, \frac{\ell_{\max}}{2}\Bigg).
$$
\end{lemma}

\paragraph{ \textbf{Proof of Theorem~\ref{thm:onl-upper}.}}
\begin{proof}
Comparing the makespan upper bound of our online algorithm (from Lemma~\ref{bdInTermstmax}) with OPT (from Lemma~\ref{lem:opt-lower}), we get that our online algorithm is $O(d +  \min\{\log t_{\max}, \log |V| \})$-competitive. The main theorem of this section is thus proved.
\end{proof}



==> logjobs.tex <==
\section{Hardness of $o( ( \log |V| )^\alpha )$-Factor Approximation for the Offline Problem}

To obtain hardness of $o( ( \log |V| )^\alpha )$-factor approximation rather than $o( ( \log t_{max} )^\alpha )$-factor approximation, we look deeper into how the LTS hardness results in \cite{LTSnotAPX} were obtained.




